Correct-by-Design Teamwork Plans for Multi-Agent Systems

We propose Teamwork Synthesis, a version of the distributed synthesis problem with application to teamwork multi-agent systems. We reformulate the distributed synthesis question by dropping the fixed interaction architecture among agents as input to the problem. Instead, our synthesis engine tries to realise the goal given the initial specifications; otherwise it automatically introduces minimal interactions among agents to ensure distribution. Thus, teamwork synthesis mitigates a key difficulty in deciding algorithmically how agents should interact so that each obtains the required information to fulfil its goal. We show how to apply teamwork synthesis to provide a distributed solution.

==> tex/toread.tex <==
% !TEX root = ../aamas23.tex
\section{to read}\label{sec:read }

\begin{definition}[Interface] Given the set of state variables $V$ of an agent, where the sets $C$, $P$, and $O$ form proper partitions of $V$, we define an interface with the form $\rulename{Int}=\conf{C,\ P,\ O}$. Intuitively, an interface partitions the state variables of an agent into three sets, each controlled by a specific component:
\begin{itemize}
\item $C$ is controlled by the context environment (nondeterministic). That is, $C$ encodes the sudden changes (or inputs) from the observable part of the execution context in which the agent operates. Thus $C$ is considered adversary and the agent cannot restrict $C$.

\item $P$ is controlled by the interaction environment. That is, $P$ encodes changes due to interactions among team members. The interaction environment is deterministic.

\item $O$ is controlled by the agent (controllable variables). That is, $O$ is a set of output variables that the agent uses to configure its state in response to inputs from both the context and the interaction environment.
\end{itemize}

\end{definition}

From the shadow TS point of view both $C$ and $P$ are input variables (i.e., $I=C\uplus P$) and only $O$ are output variables. Intuitively, we choose the interaction mode between the agent and the two environments as follows: the context environment nondeterministically enables an events from $\Exp{C}$ and the agent immediately responds to that event with a shadow transition that sets its own $O$ variables appropriately and may initiate an interaction protocol with other team members. If the response to a $C$-event incurs interaction then the control is transferred from the context environment to the interaction environment. The latter executes a finite deterministic protocol on $P$ events that the agent has to respond to appropriately by setting its $O$ variables using shadow transitions. 

The interaction environment can only execute for a finite time and eventually yields the control back to the context environment. We provide a natural execution assumption in which both the context and the interaction environments can initiate and execute a sequence of events without flooding or delaying each other indefinitely. The agent has to merely respond to events from either environments  by setting its output variables appropriately. Namely,  the interaction environment has the ability to block the context environment execution for a finite time, this is akin to the interaction environment stating that the interaction protocol is not finished yet. However, when the interaction environment yields the control back to the context, it has to yield completely, i.e., the context must have the ability to enable any event from  $\Exp{C}$. Furthermore, the interaction environment can choose to yield control immediately and thus allowing the context to execute a sequence of events. Note that the difference here with respect to RTC control \cite{rtc} is that the interaction environment is infinitely faster than the context environment. Indeed, when the control is held by the context environment, it can enable at most one event before it yields the control back to the interaction environment. The latter has the ability to yield immediately when interaction is not needed, and thus allowing the former to progress.
